Optimizing Diffusion Models for Joint Trajectory Prediction and Controllable Generation

Diffusion models are promising for joint trajectory prediction and controllable generation in autonomous driving, but they face challenges of inefficient inference steps and high computational demands. To tackle these challenges, we introduce Optimal Gaussian Diffusion (OGD) and Estimated Clean Manifold (ECM) Guidance. OGD optimizes the prior distribution for a small diffusion time $T$ and starts the reverse diffusion process from it. ECM directly injects guidance gradients to the estimated clean manifold, eliminating extensive gradient backpropagation throughout the network. Our methodology streamlines the generative process, enabling practical applications with reduced computational overhead. Experimental validation on the large-scale Argoverse 2 dataset demonstrates our approach's superior performance, offering a viable solution for computationally efficient, high-quality joint trajectory prediction and controllable generation for autonomous driving. Our project webpage is at https://yixiaowang7.github.io/OptTrajDiff_Page/.

==> config/acronyms.tex <==
\newacronym{SGD}{\textsc{sgd}}{stochastic gradient descent}
\newacronym{MAP}{\textsc{map}}{maximum-a-posteriori}
\newacronym{MLE}{\textsc{mle}}{maximum likelihood estimation}
\newacronym{MNLL}{\textsc{mnll}}{mean negative log-likelihood}
\newacronym{NLL}{\textsc{nll}}{negative log-likelihood}
\newacronym{LL}{\textsc{ll}}{log-likelihood}
\newacronym{RMSE}{\textsc{rmse}}{root mean square error}
\newacronym{ECE}{\textsc{ece}}{expected calibration error}
\newacronym{SNR}{\textsc{snr}}{signal-to-noise ratio}
\newacronym{FID}{\textsc{fid}}{Fr\'echet Inception Distance}
\newacronym{BPD}{\textsc{bpd}}{bit per dimension}
\newacronym{NFE}{\textsc{nfe}}{neural function evaluations}

\newacronym{AE}{\textsc{ae}}{auto-encoder}
\newacronym{WAE}{\textsc{wae}}{Wasserstein Auto-encoder}
\newacronym{VAE}{\textsc{vae}}{Variational Auto-encoder}
\newacronym{BAE}{\textsc{bae}}{Bayesian Auto-encoder}
\newacronym{CDF}{\textsc{cdf}}{cumulative density function}
\newacronym{GAN}{\textsc{gan}}{Generative Adversarial Network}
\newacronym{DPGMM}{\textsc{dpgmm}}{Dirichlet process Gaussian mixture model}
\newacronym{GMM}{\textsc{gmm}}{Gaussian mixture model}

\newacronym{MC}{mc}{Monte Carlo}
\newacronym{SDE}{\textsc{sde}}{Stochastic Differential Equation}
\newacronym{CNF}{cnf}{Continuous Normaxlizing Flow}
\newacronym{ODE}{ode}{Ordinary Differential Equation}
\newacronym{MCMC}{\textsc{mcmc}}{Markov chain Monte Carlo}
\newacronym{HMC}{\textsc{hmc}}{Hamiltonian Monte Carlo}
\newacronym{MH}{mh}{Metropolis-Hastings}
\newacronym{NUTS}{nuts}{no-u-turn sampler}
\newacronym{SGHMC}{\textsc{sghmc}}{stochastic gradient Hamiltonian Monte Carlo}

% \newacronym{GP}{gp}{Gaussian process}
\newacronym[longplural=deep Gaussian processes]{DGP}{\textsc{dgp}}{deep Gaussian process} % use glspl for plural
\newacronym{GPLVM}{gplvm}{Gaussian process latent variable model}
\newacronym{DPMM}{dpmm}{Dirichlet Process Mixture Model}

\newacronym{VFE}{vfe}{variational free energy}

\newacronym[longplural=Gaussian Processes]{GP}{\textsc{gp}}{Gaussian Process}
%\newacronym[plural=dgp\textnormal{s}, firstplural=Deep Gaussian Processes]{DGP}{dgp}{Deep Gaussian Process}

\newacronym{VI}{\textsc{vi}}{variational inference}
\newacronym{SVI}{\textsc{svi}}{stochastic variational inference}

\newacronym{ELBO}{\textsc{elbo}}{evidence lower bound}
\newacronym{NELBO}{\textsc{nelbo}}{negative evidence lower bound}
\newacronym{ELL}{\textsc{ell}}{expected log likelihood}
\newacronym{KL}{\textsc{kl}}{Kullback-Leibler}
\newacronym{AUC}{auc}{area under the curve}

\newacronym{BNN}{\textsc{bnn}}{Bayesian neural network}
\newacronym{DNN}{\textsc{dnn}}{deep neural network}
\newacronym{CNN}{\textsc{cnn}}{convolutional neural network}
\newacronym{MLP}{\textsc{mlp}}{multilayer perceptron}
\newacronym{NN}{nn}{neural network}
\newacronym{RELU}{ReLU}{rectified linear unit}

\newacronym{NF}{nf}{normalizing flow}

\newacronym{RBF}{rbf}{radial basis function}
\newacronym{ARD}{ard}{automatic relevance determination}

\newacronym{RKHS}{rkhs}{reproducing kernel Hilbert space}

\newacronym{OT}{ot}{optimal transport}
\newacronym{WD}{wd}{Wasserstein distance}
\newacronym{SWD}{swd}{sliced-Wasserstein distance}
\newacronym{DSWD}{dswd}{distributional sliced-Wasserstein distance}


==> table/comparison_of_realism_and_guidance_effectiveness.tex <==
\begin{table*}[h]
  \label{tb: ecmr comparison}
  \centering
  % \renewcommand\arraystretch{1.0}
% \setlength{\tabcolsep}{3pt}
	\begin{center}
 \caption{Quantitative results compared with recent methods on dataset. }
  \label{table:occ_res}
  \begin{tabular}{cc cc c cc}
\toprule
\multirow{2}*{\textbf{Setting}} & \multirow{2}*{\textbf{Method}} &\multicolumn{2}{c}{\textbf{Guidance Effectiveness}}& &\multicolumn{2}{c}{\textbf{Realism}}\\
\cmidrule{3-4}  \cmidrule{6-7}
 & & minJFDE $\downarrow$ & meanJFDE $\downarrow$ & &minJRDE $\downarrow$ & meanJRDE $\downarrow$ \\ 


 
 \midrule
 \multirowcell{5}{\textbf{Goal}} 
& No Guid & 0.808 & 3.138 &&0.164 &0.472 \\
& NNM \cite{janner2022planning, zhong2023guided} & 0.193 & 1.080 &&0.134&0.302 \\
& SF \cite{rempe2023trace,jiang2023motiondiffuser} & 0.116 & 0.633 &&0.114&0.242 \\
\cmidrule{2-7}
& ECM (Ours) & 0.056 & 0.209 &&0.113&0.232 \\
& ECMR (Ours) & 0.046 & 0.137 &&0.116&0.187 \\




\midrule
 \multirowcell{5}{\textbf{Goal\_5s}} 
& No Guid & 1.487 & 4.654 &&0.164&0.472 \\
& NNM \cite{janner2022planning, zhong2023guided}
 & 0.620 & 2.266 &&0.138&0.296 \\
& SF \cite{rempe2023trace,jiang2023motiondiffuser}
 & 0.118 & 0.872 &&0.134&0.249 \\
 \cmidrule{2-7}
& ECM (Ours) & 0.072 & 0.237 &&0.128&0.236 \\
& ECMR (Ours) & 0.061 & 0.167 &&0.131&0.195 \\





\midrule
 \multirowcell{5}{\textbf{Goal\_at5s}} 
& No Guid & 2.145 & 4.748 &&0.129&0.325 \\
& NNM \cite{janner2022planning, zhong2023guided}
 & 0.195 & 1.076 &&0.144&0.244 \\
& SF \cite{rempe2023trace,jiang2023motiondiffuser}
 & 0.160 & 1.079 &&0.140&0.275 \\
\cmidrule{2-7}
& ECM (Ours)& 0.116 & 0.457 &&0.134&0.214 \\
& ECMR (Ours)& 0.116 & 0.310 &&0.137&0.206\\




\midrule
 \multirowcell{5}{\textbf{RG}} 
& No Guid & 1.234 & 4.043 &&0.138&0.469 \\
& NNM \cite{janner2022planning, zhong2023guided}
 & 0.319 & 1.532 &&0.106&0.288 \\
& SF \cite{rempe2023trace,jiang2023motiondiffuser}
 & 0.159 & 1.041 &&0.090&0.240 \\
\cmidrule{2-7}
& ECM (Ours)& 0.061 & 0.214 &&0.088&0.208 \\
& ECMR (Ours)& 0.011 & 0.017 &&0.030&0.033\\




\midrule
 \multirowcell{5}{\textbf{RG\_5s}} 
& No Guid & 1.772 & 5.172 &&0.138&0.469 \\
& NNM \cite{janner2022planning, zhong2023guided}
 & 0.724 & 2.532 &&0.119&0.280 \\
& SF \cite{rempe2023trace,jiang2023motiondiffuser}
 & 0.155 & 1.173 &&0.126&0.249 \\
\cmidrule{2-7}
& ECM (Ours)& 0.075 & 0.244 &&0.116&0.217 \\
& ECMR (Ours)& 0.053 & 0.146 &&0.110&0.154\\




\midrule
 \multirowcell{5}{\textbf{RG\_at5s}} 
& No Guid & 2.696 & 5.575 &&0.106&0.307 \\
& NNM \cite{janner2022planning, zhong2023guided}
 & 0.275 & 1.363 &&0.132&0.231 \\
& SF \cite{rempe2023trace,jiang2023motiondiffuser}
 & 0.206 & 1.501 &&0.130&0.271 \\
\cmidrule{2-7}
& ECM (Ours)& 0.125 & 0.464 &&0.128&0.219 \\
& ECMR (Ours)& 0.106 & 0.273 &&0.118&0.170\\
\bottomrule
  \end{tabular}
  \end{center}
\end{table*}




% \begin{table*}[h]
%   \centering
%   % \renewcommand\arraystretch{1.0}
% \setlength{\tabcolsep}{3pt}
% 	\begin{center}
%  \caption{Quantitative results compared with recent methods on dataset. }
%   \label{table:occ_res}
%   \begin{tabular}{cc cc c cc}
% \toprule
% \multirow{2}*{\textbf{Setting}} & \multirow{2}*{\textbf{Method}} &\multicolumn{2}{c}{\textbf{Guidance Effectiveness}}& &\multicolumn{2}{c}{\textbf{Realism}}\\
% \cmidrule{3-4}  \cmidrule{6-7}
%  & & minJFDE $\downarrow$ & meanJFDE $\downarrow$ & &minJRDE $\downarrow$ & meanJRDE $\downarrow$ \\  
%  \midrule
%  \multirowcell{5}{\textbf{Goal}} 
% & No Guid & - & - &&- &- \\
% & NNM \cite{janner2022planning, zhong2023guided} & 0.193 & 1.080 &&0.134&0.302 \\
% % & CS \cite{rempe2023trace} & 0.32 & 0.83 &&0.26&1.15 \\
% & SF \cite{rempe2023trace,jiang2023motiondiffuser} & 0.116 & 0.633 &&0.114&0.242 \\
% \cmidrule{2-7}
% & ECM (Ours) & 0.056 & 0.209 &&0.113&0.232 \\
% & ECMM (Ours) & 0.261 & \textbf{0.414} &&\textbf{0.045}&\textbf{0.137} \\
% \midrule
%  \multirowcell{5}{\textbf{Medium}} 
% & No Guid & 0.860 & 1.881 &&1.856&4.639 \\
% & NNM \cite{janner2022planning, zhong2023guided}
%  & 0.550 & 1.098 &&0.370&1.124 \\
% % & CS \cite{rempe2023trace}
% %  & 0.42 & 0.92&&0.52&1.48 \\
% & SF \cite{rempe2023trace,jiang2023motiondiffuser}
%  & 0.427 & 0.888 &&0.448&1.217 \\
%  \cmidrule{2-7}
% & ECM (Ours) & \underline{0.391} & \underline{0.723} &&\underline{0.197}&\underline{0.425} \\
% & ECMM (Ours)& \textbf{0.340} & \textbf{0.482} &&\textbf{0.144}&\textbf{0.297} \\
% \midrule
%  \multirowcell{5}{\textbf{Hard}} 
% & No Guid & 3.680 & 4.693 &&7.198&9.919 \\
% & NNM \cite{janner2022planning, zhong2023guided}
%  & 2.080 & 3.103 &&0.935&2.694 \\
% % & CS \cite{rempe2023trace}
% %  & 0.42 & 0.92 &&0.52&1.48 \\
% & SF \cite{rempe2023trace,jiang2023motiondiffuser}
%  & 1.943 & 2.965 &&2.040&4.657 \\
% \cmidrule{2-7}
% & ECM (Ours)& \underline{1.591} & \underline{2.406} &&\textbf{0.416}&\textbf{1.014} \\
% & ECMM (Ours)& \textbf{1.507} & \textbf{2.199} &&\underline{0.445}&\underline{1.015} \\
% % & ECMMO & \textbf{0.32} & \underline{0.56} &&\textbf{0.40}&\underline{0.87} \\
% \bottomrule
%   \end{tabular}
%   \end{center}
% \end{table*}
